Towards out of equilibrium impurity solver for the Dynamical Mean Field Theory

The Dynamical Mean Field Theory (DMFT) is a powerful tool for calculating highly correlated systems (both bosonic and fermionic) in a state of thermodynamic equilibrium. However, in the case of non-equilibrium states, the method has significant limitations that do not allow obtaining correct results. The stumbling block here is the impurity solver: a method for calculating the dynamics of an open system. In this work we present the prototype of a universal impurity solver for the DMFT method which can solve both equilibrium and non-equilibrium problems. We analyse spectral functions of Bose-Hubbard model on the Bethe lattice in different regimes and show that our solver gives correct and physical results.

==> main_rus.tex <==
%\documentclass[a4paper]{article}
\input{style.tex} 
%\usepackage{braket}
%\usepackage{physics}
\graphicspath{ {./pic/} {:/pic/note1/}}
%\usepackage[small]{titlesec}
%\usepackage{indentfirst}
%\usepackage[unicode, pdftex]{hyperref}

\begin{document}
\setlength{\parindent}{1.25cm} 
% убираем висячие строки  и подобное безобразие
\sloppy   
% Запрещаем разрыв страницы после первой строки абзаца
\clubpenalty=10000		
% Запрещаем разрыв страницы перед последней строкой абзаца
\widowpenalty=10000		

% Полуторный интервал
\onehalfspacing 

\section{Введение}
Развитие таких методов, как pump-probe спектроскопия, позволило изучать временную эволюцию на масштабах электронных движений\cite{Wall_2010}\cite{Sentef_2013}. Возбуждая систему ультракороткими импульсами и затем зондируя "пробирующим" импульсом, мы можем наблюдать процесс релаксации к термодинамическому равновесию. В то время как квантовые системы в термодинамическом равновесии хорошо описываются статистической механикой, описание неравновесных систем сталкивается со множеством технических и фундаментальных проблем. 
Процесс перехода системы к стабильному состоянию после внешнего возбуждения -- это неравновесный процесс, по другому называемый термализацией. Большинство систем термализуются и в процессе релаксации теряют информацию о своём начальном состоянии, однако существуют такие явления и состояния вещества, для которых этот принцип нарушается. К примеру, это системы с многочастичной локализацией (en: many body localization или MBL)\cite{Abanin_2019}, аномальные изоляторы Флоке\cite{Rudner_2019}, аномальные нетепловые состояния в Ридберговских атомах \cite{Serbyn_2021} и многое другое

Изучение таких явлений особенно актуально в наши дни. Во-первых, это поднимает фундаментальные вопросы в термодинамике, например, о том как микроскопическая динамика приводит к термодинамическому равновесию. Во-вторых, изучение систем, подобных MBL, может открыть возможности для создания состояний, устойчивых к декогеренции, что особенно актуально в квантовых вычислениях. Поэтому сейчас активно развиваются численные подходы к моделированию неравновесной динамики. Одним из таких является неравновесная теория динамического среднего поля \cite{Aoki_2014}.

Динамическая теория среднего поля является наиболее известным численным методом в изучении сильно коррелированных фермионов или бозонов.
Ключевая идея данного метода состоит в том, что мы отображаем нашу многочастичную задачу на задачу взаимодействия квантовой примеси с внешним самосогласованным полем. 
Главную роль в данном методе играет примесный солвер (en: impurity solver), который отвечает за решение примесной задачи. Такая задача, по сути, открытой системой. Современные солверы больше подходят для фермионных систем, находящихся в равновесии \cite{Kotliar_2004}.
Равновесные бозонные системы также разрешимы, но требуют
модификации классического цикла DMFT\cite{Byczuk_2008}. 
Однако в неравновесном случае уравнения DMFT становятся сложнее, и возникают существенные ограничения, из-за которых на данный момент не существует полноценного неравновесного примесного солвера\cite{Aoki_2014}.

\begin{figure}[h!]
\center{\includegraphics[width=0.9\linewidth]{pic/DMFT_cycle_eng.png}}
%2colourlogo}}
\label{fig:DMFT}
\caption{The conception of DMFT}
\end{figure}

В данной работе мы, основываясь на концептуально новом подходе к расчету нестационарных возмущений открытых систем\cite{Polyakov_2022}, предлагаем метод решения примесной задачи в теории динамического среднего поля, подходящий как для равновесных, так и для неравновесных случаев. Наш подход является многообещающим, поскольку снижает сложность вычислений на больших временах за счёт использования границы Либа-Робинсона (аналога светового конуса в физике конденсированного состояния) \cite{SIMS_2011} в качестве критерия отбора эффективных мод внешнего окружения.
Оказывается, что в следствие обратимости временной эволюции в квантовой механике, помимо прямого светового конуса Либа-Робинсона, мы можем построить обратный. Пересечение этих конусов даёт нам обоснованный критерий для отбора мод окружения, с которыми взаимодействует примесь.
В частности, это позволяет вычислять цикл DMFT в реальном времени без неточной процедуры аналитического продолжения.

Мы проверяем корректность нашего солвера на примере расчёта спектральных функций модели Бозе-Хаббарда на решётке Бете и показывает, что наш солвер даёт физические результаты. Мы рассчитываем корреляционные функции на большом интервале времени и показываем, что для режима с отсутствием взаимодействия ($U=0$) результаты совпадают с точным решением.

\section{Метод приближенной оценки световых конусов}
В этой работе мы используем метод, который был предложен в работах \cite{Polyakov_2022}\cite{Polyakov_jan2022}. В дальнейшем для простоты мы будем называть его "методом светового конуса".

За счёт физического критерия мы можем ограничить количество мод окружения таким образом, чтобы оно оставалось фиксированным на протяжении временной эволюции системы. 
В результате получается, что открытая система взаимодействует лишь с эффективными модами, а не с полным окружением. 
Это позволяет преодолевать трудности, связанные с экспоненциальном ростом Гильбертова пространства при расчётах неравновесной динамики на больших временах. 

В своём идейном смысле метод светового конуса представляет собой ренормгруппу. Примерами подобных методов является NRG\cite{Wilson_1975}\cite{Bulla_2008} и DMRG\cite{White_1993}\cite{Kumar_2016}.
Подход ренормгруппы позволяет нам найти такое отображение исходного гамильтониана (или действия), после которого можно выделить существенные и  несущественные степени свободы (состояния), необходимые для описания системы. Например, в методе NRG отсекаются состояния с большой энергией, что позволяет сохранять размерность гильбертова пространства постоянной при добавления нового узла к цепочке. По аналогии в равновесной термодинамике каноническая матрица плотности Гиббса $\hat\rho = \exp(-\beta \hat H)$ a priori задаёт статистически значимы уровни энергии за счёт конечной температуры.
Метод светового конуса тоже производит отсечение нерелевантных состояний, но в случае временной эволюции системы. Давайте подробнее рассмотрим этот процесс.

Пусть мы работаем с системой вида:
\begin{equation}
    \hat H = \hat H_0 + \hat H_{bath} + \hat H_{int},
\end{equation}

де  $\hat H_0$, $\hat H_{bath}$ описывают подсистему и окружение соответственно, а $\hat H_{int}$ -- гамильтониан их взаимодействия. И пусть окружение описывается непрерывным спектром:
\begin{equation}
    \hat H_{bath} = \int_0^{\infty} dw w \hat b^{\dag}(w) \hat b(w),
    \label{eq:H_E}
\end{equation}
подсистема записывается как:
\begin{equation}
    \hat H_0 = \varepsilon_0 \hat b^{\dag}_0 \hat b_0,
    \label{eq:H_S}
\end{equation}
а их взаимодействие представляется в виде:
\begin{equation}
    \hat H_{int} = \hat b_0 * \int_0^{\infty} dw c(w) \hat b(w) + \hat b_0^{\dag} * \int_0^{\infty} dw c(w) \hat b^{\dag}(w).
    \label{eq:H_int}
\end{equation}
Представление в виде (\ref{eq:H_E}), (\ref{eq:H_S}) и (\ref{eq:H_int})-- это, так называемое представление открытой системы в виде "звезда"\ . От такого представления после дискретизации мы можем перейти к представлению гамильтониана системы в виде цепочки \cite{Chin_2010}, где нулевой узел отвечает примеси:
\begin{equation}
    \hat H = \varepsilon_0 \hat b^{\dag}_0 \hat b_0 + (h_0 \hat b_0^{\dag} \hat{b}_1 + c.c.) + \underbrace{\sum^{\infty}_{k=1} h_k(\hat{b}^{\dag}_{k} \hat{b}_{k+1} + c.c.) + \sum^{\infty}_{k=1} \varepsilon_k \hat{b}^{\dag}_k \hat{b}_k}_{\hat H_{bath}}.
\end{equation}

Перейдя в представление взаимодействия, мы можем исключить окружение $\hat H_{bath}$ из полного гамильтониана, при этом:
\begin{equation}
    \hat H(t) = e^{it \hat H_{bath}} \hat H e^{-it \hat H_{bath}} - \hat H_{bath},
    \label{eq:int_pic}
\end{equation}
\begin{equation}
    \hat a_1(t) = e^{i t \hat H_{bath}} \hat a_1 e^{-i t  \hat H_{bath}}.
\end{equation}

\subsection{Цикл DMFT для решётки Бете}
В случае решётки Бете в континуальном пределе числа связей ($Z\longrightarrow\infty$) цикл DMFT можно значительное упростить. Главной особенностью является тот факт, что условия согласования уравнений DMFT приобретает простой вид:
\begin{equation}
    \Delta(\omega) = t^2 G(\omega).
    \label{eq:delta}
\end{equation}

В результате весь цикл DMFT сводится к последовательности следующих операций:

0. Задать начальное приближение для локальной гриновской функции $G(\omega)$. Например, гриновской функцией для невзаимодействующей системы ($U=0$);

1. Рассчитать гибридизацию $\Delta(\omega)$ по формуле (\ref{eq:delta});

2. Решить примесную задачу и рассчитать $G_{imp}(\omega)$;

3. $G = G_{imp}$.

4. Повторить пункты 1-3 до сходимости.

\section{Решение примесной задачи}
Отображение на решение примесной задачи (пункт 2 цикла DMFT) приведено в секции 3.2 Постановка задачи. Из передаваемой функции гибридизации по формуле (\ref{c_w_i}) мы находим коэффициенты $c(w)$. После чего отобразив систему на линейную цепочку, мы приходим к гамильтониану (\ref{eq:H_imp}). В представлении взаимодействия (\ref{eq:int_pic}) полученный гамильтониан записывается в виде:
\begin{equation}
    \hat H_{imp}(t) = \hat H_0 + (h_0 \hat b^{\dag}_0 \hat b_1 + c.c.),
\end{equation}
где
\begin{equation}
    \hat b_1(t) = e^{i t \hat H_{bath}} \hat b_1 e^{-i t  \hat H_{bath}}.
\end{equation}

Далее мы полагаем, что окружение находится в термодинамическом равновесии в состоянии $\frac{1}{Z} e^{-\beta \hat H_{bath}}$. Здесь $\beta =\frac{1}{T}$ характеризует температуру окружения. В момент времени $t=0$ мы добавляем примесь к исходному окружению. Общее состояние системы в этот момент записывается как:
\begin{equation}
    \hat \rho_0(0) = \ket{0}\bra{0}_{imp} \otimes \frac{1}{Z} e^{-\beta \hat H_{bath}}.
\end{equation}

Метод светового конуса рассчитывает эволюцию этого состояния с течением времени:
\begin{equation}
    \hat \rho_0(t) = U(t) \hat \rho_0(0) U^{\dag}(t),
\end{equation}
где $U(t)=\mathcal{T} e^{-i\int_0^{t}d\tau \hat H_{imp}(\tau)}$, $\mathcal{T}$--временное упорядочивание.

Пусть $t_{0}$-- время установления равновесия в системе после добавления примеси. В результате мы имеем:
\begin{equation}
    G_{imp}(t) = -i(\langle\hat b_0(t+t_{0}) \hat b^{\dag}_0(t_{0})\rangle - \langle\hat b^{\dag}_0(t+t_{0}) \hat b_0(t_{0})\rangle),
\end{equation}
где средние:
\begin{equation}
    \langle\hat b_0(t+t_{0}) \hat b^{\dag}_0(t_{0})\rangle = Tr\{\hat b_0 U(t+t_0) \hat b^{\dag}_0 \hat\rho_0(0) U^{\dag}(t+t_0)\},
\end{equation}
\begin{equation}
    \langle \hat b^{\dag}_0(t+t_{0})\hat b_0(t_{0})\rangle = Tr\{\hat b^{\dag}_0 U(t+t_0) \hat b_0 \hat\rho_0(0) U^{\dag}(t+t_0)\}
\end{equation}
вычисляются по методу светового конуса.
\end{document}
